Incremental Training of a Detector Using Online Sparse Eigen-decomposition

The ability to efficiently and accurately detect objects plays a very crucial role for many computer vision tasks. Recently, offline object detectors have shown a tremendous success. However, one major drawback of offline techniques is that a complete set of training data has to be collected beforehand. In addition, once learned, an offline detector can not make use of newly arriving data. To alleviate these drawbacks, online learning has been adopted with the following objectives: (1) the technique should be computationally and storage efficient; (2) the updated classifier must maintain its high classification accuracy. In this paper, we propose an effective and efficient framework for learning an adaptive online greedy sparse linear discriminant analysis (GSLDA) model. Unlike many existing online boosting detectors, which usually apply exponential or logistic loss, our online algorithm makes use of LDA's learning criterion that not only aims to maximize the class-separation criterion but also incorporates the asymmetrical property of training data distributions. We provide a better alternative for online boosting algorithms in the context of training a visual object detector. We demonstrate the robustness and efficiency of our methods on handwriting digit and face data sets. Our results confirm that object detection tasks benefit significantly when trained in an online manner.

==> alg_gslda.tex <==

%
%
% GSLDA
%
%
\SetVline
\linesnumbered

\begin{algorithm}[t]
\caption{The training procedure for building an offline GSLDA object detector.}
\begin{algorithmic}
%\normalsize{
\small{
%\footnotesize{
   \KwIn{
   \begin{itemize}
      \item
         A positive training set and a negative training set;
      \item
         A set of features $\left\{f_i; i \in [1, M]\right\}$;
   \end{itemize}
   }
   
   
   \KwOut{
\begin{itemize}
   \item
      A set of selected weak learners $\left\{h_i; i \in [1, T]\right\}$ 
      that best separates the training set;
\end{itemize}
}

   
\ForEach{feature}
{
  Train a weak learner (\eg,
  a decision stump parameterized by a threshold        
  %
  % $ \theta $ 
  %
  that results in the smallest classification error) 
  on the training set;
}
   
   
\While{ the target goal is not met }
{
  Add the best weak learner (\eg, decision stump) that yields 
  the maximum class separation to the set of selected weak learners;
}

} % End \small
%
\end{algorithmic}
\label{ALG:GSLDA}
\end{algorithm}







==> alg_ogslda.tex <==

%
%
% GSLDA
%
%
\SetKwInput{KwGiven}{Given}

\SetVline
\linesnumbered

\begin{algorithm}[t]
\caption{The online GSLDA Algorithm.}
\begin{algorithmic}
%\normalsize{
\small{
%\footnotesize{
  \KwGiven{
   \begin{itemize}
      \item
         The initial set of weak learners $\left\{h_i; i \in [1, T]\right\}$ 
         trained using offline GSLDA on small initial data;
   \end{itemize}
   }


   \KwIn{
   \begin{itemize}
      \item
         New training datum $I$ and its corresponding class 
         label $y \in \left\{1,2\right\}$;
      \item
         The current between-class covariance matrix, $S_b$;
      \item
         The inverse of within-class covariance matrix, $S_w^{-1}$;
   \end{itemize}
   }
   
   
   \KwOut{
\begin{itemize}
      \item
         The updated between-class covariance matrix, $\tilde{S}_b$;
      \item
         The updated inverse of within-class covariance matrix, 
         $\tilde{S}_w^{-1}$;
      \item
         The updated weak learners' coefficients, $\tilde{\bw}$;
      \item
         The classifier threshold, $\tilde{w}_0$
   \end{itemize}
   }
   
   Classify the new datum $I$ using the given weak learners, 
      $\bx = [h_1(I), h_2(I), \cdots, h_T(I)]$; \\
   Update $S_b$ with $\bx$ using \eqref{EQ:Sb2} and~\eqref{EQ:mtilde}; \\
   Update $S_w^{-1}$ using \eqref{EQ:Sw_inv}; \\
   Recalculate weak learners' coefficients, $\bw$, using \eqref{EQ:FDA}; \\
   Update classifier threshold, $w_0$, based on node learning goal 
   (\eqref{EQ:w0Crit1} for minimal classification error, or
   $\min($\eqref{EQ:w0Crit2}$,$\eqref{EQ:w0Crit3}$)$ for the asymmetric
   node learning goal  (see Section~\ref{sec:OGSLDA_thresh}));
} % End \small
%
\end{algorithmic}
\label{ALG:OGSLDA}
\end{algorithm}







==> bio.tex <==
% LaTeX Source
% Author:        Chunhua Shen {chhshen@gmail.com}
% Creation:      Friday 07/03/2008 11:23.
% Last Revision: Monday 09/06/2009 (Paul)



% \vspace{-2em}



\begin{IEEEbiography}{Sakrapee Paisitkriangkrai} 
        is currently pursuing Ph.D. degree at the University of New
        South  Wales, Sydney, Australia. He received the B.E. degree
        in computer engineering and M.E. degree in biomedical
        engineering from the University of New South Wales in 2003.
        His research interests include pattern recognition, image
        processing and machine learning. 
\end{IEEEbiography}



\begin{IEEEbiography}{Chunhua Shen}
        received the Ph.D. degree from School of Computer Science,
        University of Adelaide,
        Australia, in 2005.  Since Oct. 2005, he has been
        a researcher with the
        computer vision program, NICTA (National ICT Australia),
        Canberra Research Laboratory.
        He is also an adjunct research fellow at the
        Australian National University; and adjunct lecturer at the
        University of Adelaide. His main research interests include
        statistical machine learning and its applications in computer
        vision and image processing. 
\end{IEEEbiography}





\begin{IEEEbiography}{Jian Zhang} 
        (M'98-SM'04) received the Ph.D. degree in electrical
        engineering from the University College, University of New
        South Wales, Australian Defence Force Academy, Australia, in
        1997.  He is a principal researcher in NICTA, Sydney.  He is
        also a conjoint associate professor at University of New South
        Wales.
        His research interests include image/video
        processing, video surveillance and multimedia content management.
        Dr. Zhang is currently an associate editor of the IEEE
        Transactions on Circuits and Systems for Video Technology and
        the EURASIP Journal on Image and Video Processing.
   \end{IEEEbiography}


